Decoupled Graph Neural Networks for Large Dynamic Graphs

Real-world graphs, such as social networks, financial transactions, and recommendation systems, often demonstrate dynamic behavior. This phenomenon, known as graph stream, involves the dynamic changes of nodes and the emergence and disappearance of edges. To effectively capture both the structural and temporal aspects of these dynamic graphs, dynamic graph neural networks have been developed. However, existing methods are usually tailored to process either continuous-time or discrete-time dynamic graphs, and cannot be generalized from one to the other. In this paper, we propose a decoupled graph neural network for large dynamic graphs, including a unified dynamic propagation that supports efficient computation for both continuous and discrete dynamic graphs. Since graph structure-related computations are only performed during the propagation process, the prediction process for the downstream task can be trained separately without expensive graph computations, and therefore any sequence model can be plugged-in and used. As a result, our algorithm achieves exceptional scalability and expressiveness. We evaluate our algorithm on seven real-world datasets of both continuous-time and discrete-time dynamic graphs. The experimental results demonstrate that our algorithm achieves state-of-the-art performance in both kinds of dynamic graphs. Most notably, the scalability of our algorithm is well illustrated by its successful application to large graphs with up to over a billion temporal edges and over a hundred million nodes.

==> author_response.tex <==
\clearpage
\setcounter{page}{1}
\section*{Author Response}
We thank the reviewers for their insightful and constructive comments. We have carefully revised the manuscript taking into account all suggestions by the reviewers, and the major changes can be summarized as three aspects:

\begin{itemize}[leftmargin = *]
  \item \textbf{Scalability Illustrations:} (for Reviewer 1)
  
  % We explicitly introduce the scalable GNN models based on decoupled framework and illustrate the differences between our approach and existing scalable static GNN models. 
  We introduced a detailed discussion of our scalable GNN models based on a decoupled framework and highlighted the key differences between our approach compared with existing scalable static GNN models. Relevant revisions are mainly in Section~\ref{sec:method}.
  \item \textbf{Time Encoding Component:} (for Reviewer 3)
  
  % We provide a variant of our basic model, which is equipped with a temporal encoding component, and its performance results. 
  We provided a variant of our basic model that includes a time encoding component and reported its performance results. Due to the page limitation, we incorporated relevant revisions into the Appendix. Note that our method still achieves significant improvements over state-of-the-art methods even without the time encoding component.
  % even without the time encoding component, our method can still significantly outperform state-of-the-art methods empirically.
  \item \textbf{Supplementary Experiments:} (for Reviewer 1, 2 and 3)
  
  % We add experiments for time cost and parameter sensitivity, and a new baseline CAW is introduced. The experimental results demonstrate the effectiveness and superiority of our method. 
  We added new experiments to evaluate time cost and parameter sensitivity, and also introduced a new baseline CAW. The results of these experiments further demonstrate the effectiveness and superiority of our method. Relevant revisions are mainly in Section~\ref{sec:exp} and the Appendix~\cite{technical_report}.
\end{itemize}

The major revised parts were highlighted in {\revision blue} for your convenience of re-reviewing. Our responses to the major concerns of reviewers were as follows. For the sake of readability, we also presented the supplementary tables and figures in the response letter, with captions beginning with A.1.

\subsection*{Reviewer 1}
\textbf{D1:} {\em In Introduction, the motivation is good to be presented. But its contribution should be improved, i.e., how the limitations are achieved should be well presented and discussed.}

\noindent \textbf{Response: }
% Thanks for pointing out this. We revise Introduction with more presentations about how our method overcomes the limitations of existing methods. 
Thanks for pointing out this. We revised the Introduction section with more presentations about how our method overcame the limitations of existing methods. Please refer to Section~\ref{sec:intro} for details.
\newline

\noindent \textbf{D2:} {\em In Section 2 – notations, it should present the concepts with more formal definitions.}

\noindent \textbf{Response: }
Thanks for the advice. We revised Section~\ref{sec:pre} to provide more formal definitions of the variables and tasks used in this paper. We also added Table~\ref{tab_response:notations} to summarize the frequently-used notations throughout the paper. \newline
\begin{table}[t]
\caption{Summary of notations.}
  \label{tab_response:notations}
\vspace{-3mm}
\begin{tabular}{c|l}
\hline
\textbf{Notation}   & \textbf{Description}        \\ \hline
$G=(V, E)$          & the graph with node set $V$ and edge set $E$    \\
$\A, \D$            & the adjacent and degree matrix         \\
$w_{(i, j)}$        & the weight of edge $(i, j) \in E$                          \\
$N(i)$              & the neighbor set of node $i$                               \\
$d(i)$              & the degree of node $i$, $d(i) = \sum_{j \in N(i)} w_{(i, j)}$ \\
$\x$                & the feature vector                            \\
$\vpi, \epi$        & the true and estimated propagation vectors    \\
$\r$                & the estimated residual vector                 \\
$(G, S)$            & the CTDG with event set $S$                                \\
$\{G_0, ..., G_T\}$ & the DTDG with $T+1$ snapshots                                \\
$G_t$               & the graph at time/snapshot $t$                             \\
$\A_t, \D_t$        & the adjacent and degree matrix of graph $G_t$  \\
$\Y$ $(\Y_t)$       & the node label matrix of graph $G$ ($G_t$) \\\hline
\end{tabular}
\end{table}

\noindent \textbf{D3:} {\em In Section 3 – Related works, it only listed what these existing works have done, but didn’t discuss how their merits to be considered or extended in this work.}

\noindent \textbf{Response: } 
Thanks for the advice. We revised Section~\ref{sec:related_work} to include more detailed discussions about the benefits and drawbacks of previous methods, and how they influenced our work.
\newline

\noindent \textbf{D4:} {\em In Section 4, it is hard to recognize how the proposed method to deal with large dynamic graphs, and what are the key differences of this work to the existing works.}

\noindent \textbf{Response:} 
Thanks for pointing out this. Our response can be summarized into the following two points:
\begin{itemize}[leftmargin = *]
  \item At the beginning of Section~\ref{sec:method} in the revised paper, we explicitly introduced the overview of our method. We design a decoupled GNN for dynamic graphs, where the dynamic propagation and prediction process are decoupled. Specifically, we eliminate the dynamic propagation parameters from the model, leaving just the parameters of the neural network learning for the downstream task. Therefore, large-scale dynamic graphs can be learned on a single machine, indicating that our model is highly scalable.
  \item At the end of Section~\ref{sec:dynamic_propagation} in the revised paper, we presented how our method handles the two types of dynamic graphs and compared it to existing methods. We highlighted that our method is capable of simulating edge deletion on dynamic graphs and can handle the simultaneous arrival of multiple edges, which is a limitation of prior CTDG-specific methods. Additionally, we emphasized that, unlike existing DTDG-specific methods that require recalculation on each snapshot, our method avoids this by constantly tracking the changes in the embedding of all nodes on the graph. \newline
  % Compared with prior CTDG-specific methods, our method is able to simulate edge deletion on dynamic graphs and can handle the simultaneous arrival of multiple edges. Compared to existing DTDG-specific methods, we avoid recalculation on each snapshot and always keep track of the changes in the embedding of all nodes on the graph. \newline
\end{itemize}
\begin{table}[t]
\caption{Comparison of the computation time for single-epoch of training (second).}
\label{tab_response:exp_ctdg_timecost}
\begin{tabular}{c|c|c}
\hline
         & Wikipedia     & Reddit   \\ \hline
JODIE    & 10            & 78       \\
TGAT     & 147           & 764      \\
DyRep    & 12            & 93       \\
TGN      & 12            & 90       \\
CAW-N-mean & 388           & 2046     \\
CAW-N-attn & 398          & 2010      \\
ours     & 2             & 12       \\ \hline               
\end{tabular}
\end{table}
\noindent \textbf{D5:} {\em Experiment should test the efficiency of different models and solutions as this work claimed to deal with large dynamic graphs, rather than small graphs.}

\noindent \textbf{Response:} 
Thanks for the advice. We included experiments on the computation time (i.e., the forward and backward propagation time), and the results are reported in Table~\ref{tab_response:exp_ctdg_timecost}. Recall that our method contains only the parameters of the sequence learning model in the prediction process. Therefore, its time cost is significantly lower than the baselines. For TGAT~\cite{xu2020tgat} and CAW-Ns~\cite{wang2021caw}, we utilize their official implementations and default hyper-parameters. The implementation of JODIE~\cite{kumar2018jodie}, DyRep~\cite{trivedi2019dyrep} and TGN~\cite{rossi2020tgn} follows Rossi et al~\cite{rossi2020tgn}.
% Please refer to the Technical Report~\cite{technical_report} for detailed experimental settings.
% We add the experiments on the computation time (i.e., the forward and backward propagation time) and report the results in Table~\ref{tab_response:exp_ctdg_timecost}. Recall that our method contains only the parameters of the sequence learning model in the prediction process, and its time cost is far lower than baselines.

\subsection*{Reviewer 2}
\textbf{W1:} {\em Lack description of hyperparameters' setting.}

\noindent \textbf{Response:} 
Thanks for pointing out this. We included additional experimental details regarding our hyperparameter settings. Please refer to the Technical Report~\cite{technical_report} for the details. \newline
% We add more experimental details about hyperparameters' setting. Due to the page limited, we incorporate relevant revisions into the Appendix. Please refer to the Technical Report~\cite{technical_report} for the details. \newline

\noindent \textbf{W2:} {\em Lack experiments for parameter sensitivity of the algorithm on datasets.}

\noindent \textbf{Response:} 
Thanks for pointing out this. Following the advice, we added experiments on the Wikipedia dataset in the revised paper to study detailed sensitivity indices for both propagation parameters and neural network parameters. The results are presented in Figure~\ref{fig_response:params_sensitivity}. Our observations indicate that the threshold $r_{max}$ can effectively control the error of node embedding, which ultimately affects the link prediction results. By carefully designing the weight coefficient, we can remove $\alpha$'s influence on the node embedding, thereby avoiding its impact on the final results. Additionally, we discovered that increasing the number of LSTM or MLP layers does not necessarily lead to better model performance. In fact, having more than eight LSTM layers may result in overfitting due to an excessive number of parameters. \newline

\noindent \textbf{W3:} {\em Lack experiments for case study.}

\noindent \textbf{Response:} 
Thanks for pointing out this. We investigated the sensitivity of our algorithm to the threshold, weight coefficient, number of LSTM layers, and number of MLP layers. The results are shown in Figure~\ref{fig_response:params_sensitivity}.
% We evaluated the sensitivity of our method to the threshold, the weight coefficient, the number of LSTM layers and MLP layers, as shown in Figure~\ref{fig_response:params_sensitivity}.


\subsection*{Reviewer 3}
\textbf{W1:} {\em Feature propagation doesn’t include time-delta component as in TGAT/TGN,}

\noindent \textbf{Response:} 
Thanks for pointing out this. Our response can be summarized into the following two points:
\begin{itemize}[leftmargin = *]
  \item In our decoupled architecture, a node's embedding change is controlled by the threshold $r_{max}$ and can be triggered by its associated events or changes in its neighborhood. As a result, each node $u \in V$ provides feedback indicating the extent to which the change affects it as soon as the graph changes. This enables us to treat the temporal representations for each node as a description of the dynamic graph from the node's perspective. Therefore, the time difference between embedding modifications is inherently included in the temporal sequence, obviating the need for explicit time encoding.
  \item On the other hand, time encoding can be introduced as supplementary information to the temporal representation in our method. Specifically, each feedback corresponds to quantified time interval information. We included the comparison results with and without time encoding, as shown in Table~\ref{tab_response:exp_time_encoding}. We use LSTM to train the future link prediction task on the four datasets. The time encoding is combined with the temporal representation generated by propagation and fed into the LSTM model to learn the temporal pattern of the dynamic graph. Our observations indicate that while the inclusion of time encoding information does improve performance, the improvement is not significant. \newline
  % For detailed experimental settings, please refer to the Technical Report~\cite{technical_report}.  \newline
\end{itemize}
\begin{figure}[t]
\setlength{\abovecaptionskip}{1mm}
\setlength{\belowcaptionskip}{-2mm}
\begin{small}
    \centering
    \vspace{-2mm}
    %    \begin{footnotesize}
    \begin{tabular}{cc}
         \hspace{-3mm}\includegraphics[height=25mm]{./figs/wiki_rmaxs.pdf} &
         \hspace{-3.5mm}\includegraphics[height=25mm]{./figs/wiki_alphas.pdf} \\ 
            (a) The threshold $r_{max}$. & (b) The weight coefficient $\alpha$. \\
         \hspace{-3mm}\includegraphics[height=25mm]{./figs/wiki_lstmlayers.pdf} &
         \hspace{-3.5mm}\includegraphics[height=25mm]{./figs/wiki_mlplayers.pdf} \\
            (c) The number of LSTM layers. & (d) The number of MLP layers.
    \end{tabular}
    % \vspace{-2mm}
    \caption{Parameter sensitivity on Wikipedia dataset.}
    \label{fig_response:params_sensitivity}
\end{small}
\end{figure}
\begin{table}[t]
\caption{Effect of time-encoding function (TE).}
  \label{tab_response:exp_time_encoding}
\vspace{-3mm}
\setlength\tabcolsep{3pt}
\begin{tabular}{l|c|ccc}
\hline
    & AP        & \multicolumn{3}{c}{MRR} \\ \hline
    & Wikipedia & UCI-Message & Bitcoin-Alpha & Bitcoin-OTC \\ \hline
w.o. TE & 99.16     & 0.214       & 0.3405        & 0.3102      \\
w. TE   & 99.20     & 0.215       & 0.3423       & 0.3208      \\ \hline
\end{tabular}
\end{table}

\noindent \textbf{W2:} {\em Authors haven’t compared the proposed method with CAW (https://arxiv.org/abs/2101.05974)}

\noindent \textbf{Response:} 
Thanks for pointing out this. We added a brief description of the CAW method in the related work section, and we have included its results as a new baseline on the second and third rows of the bottom of Table~\ref{tab:exp_ctdg}. Please refer to Section~\ref{sec:exp_ctdg} for more details. As shown in the table, CAW is indeed a powerful baseline method. However, we found that it requires more computing time (as shown in Table~\ref{tab_response:exp_ctdg_timecost}) and cannot scale to large dynamic graphs, such as GDELT and MAG used in our paper, due to the high number of parameters. \newline
% As suggested by the reviewer, we add a brief description of CAW in related work and report the results of CAW as a new baseline on the second and third lines of Table~\ref{tab:exp_ctdg}'s bottom. Please refer to Section~\ref{sec:exp_ctdg} for details. As shown in the table, CAW is indeed a powerful baseline method. However, we found that CAW spends more time in computing (as shown in Table~\ref{tab_response:exp_ctdg_timecost}) and cannot scale to GDELT and MAG, the two large dynamic graphs used in the paper. \newline

\noindent \textbf{W3.1:} {\em Main method is bit hard to follow.}

\noindent \textbf{Response:} 
Thanks for pointing out this. We reorganized Section~\ref{sec:method} to make it more accessible for readers to follow and introduced more details of scalable GNNs and approximate propagation. \newline
% We reorganize Section~\ref{sec:method} and revise the related presentation, in order to make it easy for readers to follow. \newline

\noindent \textbf{W3.2:} {\em It seems that algorithm 1 is not the paper’s contribution, reference needs to be mentioned clearly.}

\noindent \textbf{Response:} 
Thanks for pointing out this. 
In Section~\ref{sec:method} of the revised paper, we added references and explained the improvements of our method. Specifically, we generalize dynamic propagation~\cite{zheng2022instantgnn} to weighted graphs and loosen the condition that the weight coefficients must be positive.
% is fixed to $\alpha \in (0, 1)$.



